Tight Bounds for Low Dimensional Star Stencils in the Parallel External Memory Model

Stencil computations on low dimensional grids are kernels of many scientific applications including finite difference methods used to solve partial differential equations. On typical modern computer architectures, such stencil computations are limited by the performance of the memory subsystem, namely by the bandwidth between main memory and the cache. This work considers the computation of star stencils, like the 5-point and 7-point stencil, in the external memory model and parallel external memory model and analyses the constant of the leading term of the non-compulsory I/Os. While optimizing stencil computations is an active field of research, there has been a significant gap between the lower bounds and the performance of the algorithms so far. In two dimensions, this work provides matching constants for lower and upper bounds closing a multiplicative gap of 4. In three dimensions, the bounds match up to a factor of $\sqrt{2}$ improving the known results by a factor of $2 \sqrt{3}\sqrt{B}$, where $B$ is the block (cache line) size of the external memory model. For dimensions $d\geq 4$, the lower bound is improved between a factor of $4$ and $6$. For arbitrary dimension~$d$, the first analysis of the constant of the leading term of the non-compulsory I/Os is presented. For $d\geq 3$ the lower and upper bound match up to a factor of $\sqrt[d-1]{d!}\approx \frac{d}{e}$.

==> upperBoundsLowerOrderTerms.tex <==
% \documentclass{llncs}
% 
% \usepackage{graphicx}
% \usepackage[english]{babel}
% \usepackage[latin1]{inputenc}  \usepackage[T1]{fontenc}
% \usepackage{lmodern}           	
% \usepackage{amsmath} 
% \usepackage{amssymb}
%  \usepackage{subfigure} \usepackage{lscape}
% \usepackage{tikz}
% \usetikzlibrary{decorations.pathreplacing}
% \usetikzlibrary{shapes}
% \usetikzlibrary{arrows}
% \usetikzlibrary{snakes}
% \usetikzlibrary{trees}
% \usepackage{ifthen}
% \usepackage{lscape}
% 
% 
% \usepackage{framed}
% \definecolor{shadecolor}{rgb}{1,0.8,0.3}
% 
% 
% \newcommand{\Transfer}{\textit{Transfer}}
% \newcommand{\pathwidth}{\textit{pathwidth}}
% \newcommand{\Eval}{\textit{Eval}}
% \newcommand{\mO}[1] {\mathcal{O}\left( #1 \right)}
% \newcommand{\ceil}[1] {\left\lceil #1 \right\rceil}
% \def\ac{\!\!\!\!\!\!}
% 
% 
% \begin{document}


% 		\section{Detailed Analysis of the Upper Bounds}
% 			\label{sec:upperBoundsLowerOrderTerms}
% % 
% 			The exact analysis of the lower order terms presented in this section is tedious work. The detailed analysis keeps repeating the same steps for every algorithm and is mainly bookkeeping of the different lower order terms.
% 
% 			For the detailed analysis of the upper bounds we assume that the data is given in the layout separated into core bands and wing bands such that no reordering of the data is necessary. Additionally, for each subset of working bands that share wing bands, the data is also saved in separate blocks. The number of working bands that are adjacent to each other is at most $2^n$. This and also the number of subsets of overlapping working bands solely depends on $n$. 

% 			We make intense use of the assumptions $\frac{k_i}{M}\to \infty$ for $i \in \{ 1,\, \dots \, ,\, n\}$ and $\frac{M}{B} \to \infty$ and regard everything that grows slower than the leading term of the non-compulsory I/Os as lower order terms. In particular terms that solely depend on $n$ or $s$ are regarded  constant.
% % 
% 			To account for all the I/Os that could occur during the algorithm we first derive a more complicated formula for the upper bound taking into account the difference between working band and the vertices that can be evaluated in a working band, overlap of more than two working bands, blocking the working band into several parts belonging to different intersections of wing bands, reserving blocks for the output, etc. In this first estimation we are sometimes overly pessimistic to simplify the formula for the upper bound. This formula is then simplified step by step while we keep book of all error terms that are dropped. When an error term is calculated, we summarize in parentheses what the error term accounts for.
% 
% 			When simplifying denominator of upper bounds we use the following observation:
% 			\begin{equation}\label{eq:enumeratorScheme}
% 				\frac{1}{m-a} = \frac{1}{m}+\frac{a}{m^2-ma} \; .
% 			\end{equation}
% 
% 			As the output is written in whole blocks we have to save space in internal memory to gather the results of every separately blocked intersection of wing bands. As discussed this number is constant and so, for some constant $c$, $M-cB$ spots in internal memory are left to load the input data.

			
% 
% 
% 			\subsection{Analysis of the Lower Order Terms of the Two Dimensional Row Layout}
% 					This section details the analysis of the two dimensional row layout first discussed in Sect. \ref{sec:2DLayouts}. 
% 					To ensure that only a constant number of output blocks is needed, the data is written back in block aligned column layout. Otherwise an output block would be needed for every row of the sweep shape making the number of output blocks dependent on the size of the sweep shape. This change in layout is only needed for the row layouts in two and three dimensions, as only there vertices that are evaluated consecutively are saved in different blocks. This reordering ensures that we need only $c=3$ output blocks. 
% 
% 					Now consider the input. For $B\geq 2s$ one block has to be in internal memory per row of the sweep shape. In the worst case the layout is block aligned so that the $2s$ previous sweep shapes are also needed. Since we do not need to write the vertices of the core band we reorder them in internal memory so that at most $2s\cdot (m-4s)$ have to stay in internal memory. The  $2s \cdot 4s $ vertices of the wing bands are needed to evaluate other working bands. To preserve the data layout the whole block containing the $2s$ vertices is kept in memory. This gives
% 					\begin{equation*}
% 						m\cdot B +\left(\left\lceil\frac{2s\cdot(m-4s)}{B}\right\rceil+1\right) B+4s \cdot B \leq M-cB \enspace.
% 					\end{equation*}
% 					Capturing in $c' = c+2+4s$ the effects of the additional blocks for the wing bands and core bands, this solves to
% 					\begin{equation*}
% 						m = \left\lfloor\frac{M-c'B+8s^2}{B+2s}\right\rfloor \enspace.
% 					\end{equation*}
% 					$\left\lceil\frac{k_2}{m-2s}\right\rceil$ 
% 					estimates the number of working bands. Per row there are at most $\left\lceil\frac{k_1}{B}\right\rceil +1$ blocks. Per working band each of these blocks causes an I/O for each of the $4s$ wing rows. Additionally, if the block does not end when the row ends, we need another $2m$ I/Os per working band to write and read the blocks covering two different rows. This yields an upper bound of
% 					\begin{equation*}
% 						\left\lceil\frac{k_2}{m-2s}\right\rceil
% 						\left( 2m + \left( \left\lceil\frac{k_1}{B}\right\rceil +1\right)4s\right) 
% 					\end{equation*}
% 					which we now simplify step by step collecting lower order terms. Consider the second term first.  Simplifying the second term to $\frac{k_1}{B}\cdot 4s$ yields an error term of at most 
% 					\begin{equation}
% 						\left\lceil\frac{k_2}{m-2s}\right\rceil
% 							\cdot (2m+2\cdot 4s) = \mathcal{O}\left(k_2 \right) \; .
% 							\label{eq:2DRowErrork2}
% 					\end{equation}
% 					(If every block spans two rows, there is one additional I/O per row.)
% 					Now simplifying the first term to $\frac{k_2}{m-2s}$ adds an error of about
% 					\begin{equation*}
% 						1\cdot \frac{k_1}{B}\cdot4s = \mathcal{O}\left(\frac{k_1}{B}\right) \; .
% 					\end{equation*}
% 					(Contribution of the wing rows of the last (partial) working band.)
% 					So we are left at
% 					\begin{equation*}
% 						\frac{k_2}{m-2s}\cdot \frac{k_1}{B}\cdot 4s \; .
% 					\end{equation*}
% 					By simplifying the denominator to $m$, we collect another error term of
% 					\begin{equation}
% 						k_2\cdot \frac{2s}{m^2-2ms}\cdot \frac{k_1}{B}\cdot4s = \mathcal{O}\left(k_1k_2\frac{B}{M^2} \right) %\; .
% 						\label{eq:2DRowErrorBoverM2-vers1}
% 					\end{equation}
% 					(Core band is smaller than working band	.)
% 					to arrive at 
% 					\begin{equation*}
% 						\frac{k_2}{m}\cdot \frac{k_1}{B}\cdot4s = \frac{k_2}{\left\lfloor\frac{M-c'B+8s^2}{B+2s}\right\rfloor}\cdot \frac{k_1}{B}\cdot4s \leq k_2\frac{B+2s}{M-c'B+8s^2-B-2s}\cdot \frac{k_1}{B} \cdot 4s\;.
% 					\end{equation*}
% 					First simplify the denominator to $M$, collecting
% 					\begin{equation}
% 						k_2 \cdot \frac{k_1}{B}\cdot 4s  \cdot (B+2s)\cdot\frac{c'B-8s^2+B+2s}{M^2-Mc'B+8s^2M-MB-2sM} = \mathcal{O}\left( k_1k_2\frac{B}{M^2}\right) \; . 
% 						\label{eq:2DRowErrorBoverM2-vers2}
% 					\end{equation}
% 					(Output blocks, work in full blocks.) Now simplify the enumerator to $B$ to arrive at
% 					\begin{equation*}
% 						k_2\cdot \frac{B}{M}\cdot \frac{k_1}{B}\cdot 4s = \frac{4s}{M}\cdot k_1k_2
% 					\end{equation*}
% 					collecting the last error term of
% 					\begin{equation}
% 						k_2 \cdot \frac{k_1}{B}\cdot 4s  \cdot \frac{2s}{M} = \mathcal{O}\left(\frac{k_1k_2}{BM} \right) \; .
% 						\label{eq:2DRowError1OverBM}
% 					\end{equation}
% 					($m$ blocks and $2s$ sweep shapes have to in in internal memory.) Let us sum up and simplify the error terms:
% 					\begin{equation*}
% 						\mathcal{O}\left(k_2 + \frac{k_1}{B}+k_1k_2\frac{B}{M^2}+\frac{k_1k_2}{BM} \right) = \mathcal{O}\left(k_2 + k_1k_2\frac{B}{M^2}+\frac{k_1k_2}{BM} \right)   \; .
% 					\end{equation*}
% 					This yields the final upper bound of 
% 					\begin{equation*}
% 						\frac{4s}{M}\cdot k_1k_2+\mathcal{O}\left(k_2 + k_1k_2\frac{B}{M^2}+\frac{k_1k_2}{BM} \right)  
% 						= \left(\frac{4s}{M} +\mathcal{O}\left(  \frac{1}{k_1}+\frac{B}{M^2}+\frac{1}{BM}     \right)\right) \cdot k_1k_2 \; .
% 					\end{equation*}
% % 
% 
% 
% 
% 			\subsection{Analysis of the Lower Order Terms of the Three Dimensional Row Layout}
% 
% 				The sweep shape is a square of $m$ vertices per side, lying in an $x_2x_3$ plane and shifted along $x_1$. To need only a constant number of $c=9$ output blocks the results are saved in a block aligned column layout, as in the two dimensional case. Assuming $B\geq 2s$ one block has to be in internal memory per row of the sweep shape. In the worst case of a block aligned row layout, the $2s$ previous sweep shapes are also needed. As in two dimensions, the vertices in the core band are rearranged in internal memory while the vertices of the wing bands stay in row layout when the input is written back to external memory. The core band is a square band of $m-4s$ vertices per side. The wing bands consists of $4\cdot (m-4s)\cdot 2s +4\cdot 2s\cdot 2s= 2s\cdot(m-2s)$ rows in total. They can be subdivided into two classes. There are four wing bands each when two respectively four working bands overlap. They consists of $(m-4s)\cdot 2s$ or $2s\cdot 2s$ vertices each. So $m$ has to fulfill
% 				\begin{align}
% 					m^2\cdot B &+ \left (\left\lceil \frac{2s \cdot (m-4s)^2}{B}\right\rceil +1 \right) \cdot B+ 4\cdot 2s \cdot (m-2s)\cdot B \leq M-cB \enspace.
% 					\label{eq:mBound3DRow}
% 				\end{align}
% 				Solving this quadratic equation, adding an additional $+1$ for dropping the ceiling function,  yields
% 				\begin{align*}
% 				 m_{1,\,2}&= \frac{16s^2-8sB\pm}{2\cdot(B+2s)\cdot} \dots\\
% 					&\dots \frac{\pm\sqrt{(-16s^2+8sB)^2-4(B+2s)(32s^3+2B-16s^2B-M+cB)}}{\cdot 1}
% 					\enspace.
% 				\end{align*}
% 				Since $m$ only has to suffice the upper bound from \eqref{eq:mBound3DRow} we can estimate
% 				\begin{align*}
% 					&\frac{16s^2-8sB\pm\sqrt{(-16s^2+8sB)^2-4(B+2s)(32s^3+2B-16s^2B-M+cB)}}{2\cdot(B+2s)}\geq \\ 
% 					&\geq \frac{-8sB+\sqrt{4(B+2s)(-32s^3-2B+M-cB)}}{2\cdot(B+2s)} \geq \\
% 					&\geq \frac{\sqrt{M-32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}}{\sqrt{B+2s}} 
% 					\enspace.
% 				\end{align*}
% 				So we choose
% 				\begin{equation*}
% 					m = \left\lfloor \frac{\sqrt{M-32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}}{\sqrt{B+2s}}  \right\rfloor \enspace.
% 				\end{equation*}
% 				For the analysis of the lower order terms we need the asymptotic behavior of $m$ which is $m =\mO{\sqrt{\frac{M}{B}}}$. 
% 				There are $\ceil{ \frac{k_2}{m-2s} }$ working bands in $x_2$ direction and $\ceil{\frac{k_3}{m-2s}}$ in $x_3$ direction. The wing bands that take part in two working bands cause one non-compulsory I/Os for each working band they take part in. The wing bands that take part in four working bands cause 6 non-compulsory I/Os in total. We overestimate this by 2 non-compulsory I/Os for every working band they are in. Furthermore we account for another $2m^2$ I/Os per working band to read and write the first and last block of each working band. Altogether the upper bound is
% 				\begin{equation*}
% 					\ceil{ \frac{k_2}{m-2s} }\ceil{ \frac{k_3}{m-2s} }\left(2m^2+ \left( \ceil{\frac{k_1}{B}}+1 \right)\cdot 4\cdot \left( 2s \cdot (m-4s)+ 2\cdot 2s\cdot 2s \right)\right) \enspace.
% 				\end{equation*}
% 				This is now simplified. First, dropping the first two ceiling functions yields the two error terms
% 				\begin{align*}
% 					&\ceil{\frac{k_3}{m-2s}}\cdot \left(2m^2+ \left( \ceil{\frac{k_1}{B}}+1 \right)\cdot 4\cdot \left( 2s \cdot (m-4s)+ 2\cdot 2s\cdot 2s \right)\right) = \mO{\frac{k_1k_3}{B}}\enspace \end{align*} and \begin{align*}
% 					&\frac{k_2}{m-2s}\cdot \left(2m^2+ \left( \ceil{\frac{k_1}{B}}+1 \right)\cdot 4\cdot \left( 2s \cdot (m-4s)+ 2\cdot 2s\cdot 2s \right)\right) = \mO{\frac{k_1k_2}{B}} \enspace.
% 				\end{align*}
% 				(The last, incomplete working band in both directions.)
% 				Simplifying the third term to $\frac{k_1}{B}$ adds an error of
% 				\begin{align*}
% 					\frac{k_2}{m-2s}\cdot \frac{k_3}{m-2s}\cdot \left(2m^2+ 2\cdot 4\cdot \left( 2s \cdot (m-4s)+ 2\cdot 2s\cdot 2s \right)\right) = \mO{k_2k_3} 
% 				\end{align*}
% 				(Additional I/Os for each row when blocks go over two rows and, lower order, estimating blocks per row.)
% 				such that the upper  bound reads
% 				\begin{equation*}
% 					 \frac{k_2}{m-2s} \cdot\frac{k_3}{m-2s}\cdot\frac{k_1}{B} \cdot 4\cdot \left( 2s \cdot (m-4s)+ 2\cdot 2s\cdot 2s \right)=  \frac{k_2}{m-2s}\cdot \frac{k_3}{m-2s}\cdot\frac{k_1}{B} \cdot 8ms
% 					\enspace.
% 				\end{equation*}
% 				We drop the $-2s$ terms which yields errors of
% 				\begin{align*}
% 					k_2\cdot \frac{2s}{m^2-2sm} \cdot \frac{k_3}{m-2s}\cdot\frac{k_1}{B} \cdot 8ms &= \mO{\frac{k_1k_2k_3}{M}} \enspace \mbox{and}\\
% 					\frac{k_2}{m}\cdot k_3\cdot \frac{2s}{m^2-2sm} \cdot\frac{k_1}{B} \cdot 8ms &= \mO{\frac{k_1k_2k_3}{M}} \enspace.
% 				\end{align*}
% 				(Outer wing band cannot be evaluated.)
% 				As next step we substitute the value of $m$ and get, using the concavity of the square root,
% 				\begin{align*}
% 					\frac{8 s \cdot k_1k_2k_3}{B}\cdot \frac{1}{m} = \frac{16 s \cdot k_1k_2k_3}{B}\cdot \frac{1}{\left\lfloor \frac{\sqrt{M-32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}}{\sqrt{B+2s}}  \right\rfloor} \leq \\
% 					\leq  \frac{8 s \cdot k_1k_2k_3}{B}\cdot \frac{\sqrt{B}+\sqrt{2s}}{\sqrt{M}-\sqrt{32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}-\sqrt{B+2s}} \enspace .
% 				\end{align*}
% 				Simplifying the enumerator yields an error of
% 				\begin{align*}
% 					\frac{8 s \cdot k_1k_2k_3}{B}\cdot \frac{\sqrt{2s}}{\sqrt{M}-\sqrt{32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}-\sqrt{B+2s}} = \mO{\frac{k_1k_2k_3}{B\sqrt{M}}}
% 				\end{align*}
% 				($2s$ previous sweep shapes are needed in memory.)
% 				and then simplifying the denominator
% 				\begin{align*}
% 					\frac{8 s \cdot k_1k_2k_3}{B}\cdot \sqrt{B}\cdot \frac{\sqrt{32s^3-2B-cB}+\frac{4sB}{\sqrt{B+2s}}+\sqrt{B+2s}}{M-\sqrt{M}\left(\sqrt{32s^3-2B-cB}-\frac{4sB}{\sqrt{B+2s}}-\sqrt{B+2s}\right)} &= \\
% 						& \! \! \! \! \! \! \! \! \! \! \! \! \! \! \! \!\! \! \! \! \! \! \! \!= \mO{\frac{k_1k_2k_3}{M}} \enspace.
% 				\end{align*}
% 				(Blocks for output and for each part of the core and wing bands.)
% 				Hence the number of non-compulsory I/Os is upper bounded by
% 				\begin{equation*}
% 					\frac{8 s \cdot k_1k_2k_3}{\sqrt{B}\sqrt{M}}+\mO{\frac{k_1k_2k_3}{M}+\frac{k_1k_2k_3}{B\sqrt{M}}} = \frac{k_1k_2k_3}{\sqrt{B}\sqrt{M}}\cdot \left(8s +\mO{\frac{\sqrt{B}}{\sqrt{M}}+\frac{1}{\sqrt{B}}} \right)
% 					\enspace.
% 				\end{equation*}


				
 
% \end{document}
